IDKM: Memory Efficient Neural Network Quantization via Implicit, Differentiable k-Means

Compressing large neural networks with minimal performance loss is crucial to enabling their deployment on edge devices. (Cho et al., 2022) proposed a weight quantization method that uses an attention-based clustering algorithm called differentiable $k$-means (DKM). Despite achieving state-of-the-art results, DKM's performance is constrained by its heavy memory dependency. We propose an implicit, differentiable $k$-means algorithm (IDKM), which eliminates the major memory restriction of DKM. Let $t$ be the number of $k$-means iterations, $m$ be the number of weight-vectors, and $b$ be the number of bits per cluster address. IDKM reduces the overall memory complexity of a single $k$-means layer from $\mathcal{O}(t \cdot m \cdot 2^b)$ to $\mathcal{O}( m \cdot 2^b)$. We also introduce a variant, IDKM with Jacobian-Free-Backpropagation (IDKM-JFB), for which the time complexity of the gradient calculation is independent of $t$ as well. We provide a proof of concept of our methods by showing that, under the same settings, IDKM achieves comparable performance to DKM with less compute time and less memory. We also use IDKM and IDKM-JFB to quantize a large neural network, Resnet18, on hardware where DKM cannot train at all.

==> resnet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\begin{tabular}{@{}llrr@{}}
\toprule
k  & d & \multicolumn{1}{l}{\textbf{Implicit}} & \multicolumn{1}{l}{\textbf{Implicit-JFP}} \\ \midrule
2  & 1 & 0.5292                                & \textbf{0.5346}                           \\
4  & 1 & \textbf{0.897}                        & 0.8961                                    \\
8  & 1 & \textbf{0.92844}                      & 0.92733                                   \\
2  & 2 & 0.3872                                & \textbf{0.4742}                           \\
4  & 2 & \textbf{0.897}                        & 0.8961                                    \\
16 & 4 & \multicolumn{1}{l}{tbd}               & \textbf{0.8648}                           \\ \bottomrule
\end{tabular}
\caption{Quantization results on a Resnet18 model pretrained on CIFAR10. Using the maximum number of clustering iterations allowed by our hardware, the feed-forward implementation of soft-$k$-means never outperforms random assignment and so its performance is not reported.Note that when $k=2$, the number of bits required for storage is $1$. With $k=2$ and $d=2$, half a bit is used for every weight in the quantized model.}
\label{tab:resnet}
\end{table}
